Quantum signatures of classical multifractal measures

A clear signature of classical chaoticity in the quantum regime is the fractal Weyl law, which connects the density of eigenstates to the dimension $D_0$ of the classical invariant set of open systems. Quantum systems of interest are often {\it partially} open (e.g., cavities in which trajectories are partially reflected/absorbed). In the corresponding classical systems $D_0$ is trivial (equal to the phase-space dimension), and the fractality is manifested in the (multifractal) spectrum of R\'enyi dimensions $D_q$. In this paper we investigate the effect of such multifractality on the Weyl law. Our numerical simulations in area-preserving maps show for a wide range of configurations and system sizes $M$ that (i) the Weyl law is governed by a dimension different from $D_0=2$ and (ii) the observed dimension oscillates as a function of $M$ and other relevant parameters. We propose a classical model which considers an undersampled measure of the chaotic invariant set, explains our two observations, and predicts that the Weyl law is governed by a non-trivial dimension $D_\mathrm{asymptotic} < D_0$ in the semi-classical limit $M\rightarrow\infty$.

==> response_to_reports <==
1) What is the \nu_peak? Does it have a classical meaning?

|\nu|_peak is the most probable eigenvalue and it can be approximated as the median of \rho( |\nu| ) (see Figs. 3 and 4).  Its position is proportional both to R and to the size of the leaky region. However, a simple relation of the position to, for instance, the classical escape-rate does not seem to exist.

2) Which is the dependence of the results with the width of the absorbing region?

As stated above, R and the size of the leak play a comparable role, but while a change in R and in the width both change the classical escape rate, their influence on the measure \mu is fundamentally different.
A change in R changes the amplitude of fluctuations in \mu but keeps the overall structure intact. That is, by a non-linear squeezing/stretching in \mu-direction you could make the distributions belonging to different values of R identical. 
A change of the with on the other hand also changes the spatial structure, so that such a transformation is impossible.
Since initially we were mostly interested in the transition from full to partial absorption, we did not study the influence of the width but concentrated on changes in the reflectivity. This also allowed us to compare our findings to the analytical results presented in the manuscript.


changes:

*  \nu_peak -> \nu_typ
*  changed and extended first paragraph on page 3 after "States peak around..." accordingly.
*  caption of Fig. 4 Middle Row extended (now grey-scale readable label)
*  caption of Fig. 5b changed (now grey-scale readable label)
*  caption of Fig. 7a changed (now grey-scale readable label)




In the case of the baker map the absorbing region was chosen in order to allow for comparison with analytical calculations.
In the case of the cat map we chose an arbitrary asymmetric region.
The essential point for our investigation of the role of partial opening is that both cases lead to a non-trivial D_0 for R=0.  


States concentrate around a typical value $\left|\nu\right|_{\mathrm{typ}}$, which is $\left|\nu\right|_{\mathrm{typ}}\approx0$ for $R=0$, increases with $R$, and can be approximated as the median of $\rho(\left|\nu\right|)$.


******************** Answer to the referees **************************

We'd like to thank both referees for their careful reading of our
manuscript. We are pleased that both reviewers recognize the
significance of our results and recommend publication. Below are the
answers to the two questions raised by referee #1. At the end we list
the modifications we have performed in our manuscript to address them.


Referee #1: "1) What is the \nu_peak? Does it have a classical meaning?"

|\nu|_peak is the typical lifetime of an eigenstates. It is computed as
the median of the distribution of lifetimes \rho(|\nu|) (see Figs. 3 and
4) and coincides in all cases with the peak of the \rho(|\nu|). The
value of |\nu|_peak is proportional both to R and to the size of the
leaky region. A classical quantity that share the same properties is the
escape rate of an ensemble of initial conditions. We have modified our
manuscript to clarify these issues, see point A) in the list below.


#Referee 1: "2) Which is the dependence of the results with the width of
the absorbing region?"

The width of the absorbing region controls the classical escape rate of
the system and therefore, as stated above, the distribution \rho(|\nu|)
of lifetimes of the eigenstates. In this sense, the size of the
absorbing region and the reflection coefficient R play a comparable
role. However,their influence on the measure \mu is fundamentally
different. For instance, a change in R does not change the fractal
dimension (D_0=2), while a change in the width of the absorbing region
typically does (D_0 at R=0 decreases for increasing width). Changing the width
of the absorbing region leads to different exponents in the usual
fractal Weyl law, but the law itself is independent of this choice.
Since we are mostly interested in the modifications of fractal Weyl law
for the case of partial absorption (classical multifractality), in our
manuscript we concentrated on changes in R for a fixed width. Our main
results are independent of the particular choice of the width. We have
modified our manuscript to clarify these issues, see point B) in
the list below.


*********************** Summary of changes *********************

A) Instead of |\nu|_peak we now use |\nu|_typ. The following text was added
   on page 3:

"The states concentrate around a typical value |\nu|_typ,
which is |\nu|_typ\approx 0 for R=0, increases with R,
and can be approximated as the median of \rho(|\nu|)."

B) We included a sentence on page two shortly before chapter III that
   clarifies the role of he width of the absorbing region:

"In the case of the baker map the absorbing region was chosen in order to
allow for comparison with analytical calculations.
In the case of the cat map we chose an arbitrary asymmetric region.
The essential point for our investigation of the role of partial opening
is that both cases lead to a non-trivial D_0 for R=0." 

C) We updated the caption of the figures in order to comply with the APS
   standard for "color online" figures.

*  caption of Fig. 4 Middle Row extended (grey-scale readable label)
*  caption of Fig. 5b changed (grey-scale readable label)
*  caption of Fig. 7a changed (grey-scale readable label)


